Finding the Parallels: A Path to Evaluating Summarization from Low-Resource Languages

Across benchmarks, large language models have demonstrated impressive summarization capabilities for high-resource languages. In contrast, summarization benchmarks are largely unavailable for low-resource languages. This scarcity poses a challenge for both evaluating LLM summarization capabilities and measuring the effectiveness of LLM-as-a-Judge approaches in these languages. However, previous work in machine translation has contributed parallel datasets that pair sentences in low-resource languages with higher-resource translations. We introduce ParaWeave, a method for automatically transforming these existing sentence-level parallel datasets into coherent document-level benchmarks while preserving their original cross-lingual alignment. We used ParaWeave to construct a summarization benchmark that spans ten language varieties from three families (Afro-Asiatic, Indo-Iranian, and Nilo-Saharan). We use the resulting benchmark to evaluate summarization faithfulness and LLM-as-a-Judge performance for summaries generated from documents in these languages. Pairing low-resource language documents with high-resource translations enables studying the effect of source language on both summarization quality and LLM-as-a-Judge performance. These comparisons reveal gaps in model performance and demonstrate that even current frontier models struggle with faithful low-resource language summarization and evaluation in certain languages. For example, GPT-5.5's summaries of Nilo-Saharan documents are significantly less faithful than their English document counterparts. Native-speaker annotations validate the model judgments in our construction pipeline and judge faithfulness metrics. The proposed pipeline offers a general approach for repurposing existing sentence-level parallel resources for evaluation of document-level tasks.

==> visuals.tex <==
\RequirePackage{fix-cm}
\usepackage[semibold]{sourcesanspro}
\usetikzlibrary{arrows.meta,calc,positioning,shapes.geometric,shadows,backgrounds,fit,decorations.pathreplacing}
\definecolor{cbInk}{HTML}{24353E}
\definecolor{cbMuted}{HTML}{5A6B75}
\definecolor{cbLine}{HTML}{CDD7DC}
\definecolor{cbPaper}{HTML}{F5F7F8}
\definecolor{cbBlue}{HTML}{366D9E}
\definecolor{cbBluePale}{HTML}{EAF1F8}
\definecolor{cbGold}{HTML}{91631F}
\definecolor{cbGoldPale}{HTML}{F7EEDC}
\definecolor{cbGreen}{HTML}{256B59}
\definecolor{cbGreenPale}{HTML}{E8F2ED}
\definecolor{cbAmber}{HTML}{936018}
\definecolor{cbAmberPale}{HTML}{FCF0D7}
\definecolor{cbRed}{HTML}{A04D53}
\definecolor{cbRedPale}{HTML}{F9EAEC}
\definecolor{oaiNavy}{HTML}{1F4E94}
\newcommand{\chartmono}{\ttfamily}
\ifXeTeX\else\IfFileExists{T1SourceCodePro-TLF.fd}{\renewcommand{\chartmono}{\fontencoding{T1}\fontfamily{SourceCodePro-TLF}\selectfont}}{}\fi
\tikzset{
  cbBase/.style={x=1cm,y=-1cm,font=\sffamily\fontsize{8.5}{10.5}\selectfont,
    text=cbInk,every node/.style={outer sep=0pt,inner sep=0pt}},
  cbHead/.style={anchor=west,font=\sffamily\bfseries\fontsize{9}{11}\selectfont},
  cbSmall/.style={font=\sffamily\fontsize{7.2}{9}\selectfont,text=cbMuted},
  cbTiny/.style={font=\sffamily\fontsize{6.6}{8}\selectfont,text=cbMuted},
  cbText/.style={anchor=north west,align=left},
  cbCard/.style={draw=cbLine,fill=white,line width=.55pt,rounded corners=3pt},
  cbFlow/.style={draw=cbInk!75,line width=.9pt,-{Latex[length=1.65mm,width=1.2mm]},rounded corners=3pt},
  cbRecycle/.style={cbFlow,draw=cbRed,dash pattern=on 3pt off 2pt},
  cbStep/.style={circle,fill=cbInk,text=white,minimum size=.34cm,
    font=\sffamily\bfseries\fontsize{7}{8}\selectfont},
  cbIndex/.style={circle,fill=cbPaper,draw=cbLine,line width=.45pt,
    minimum size=.32cm,font=\sffamily\fontsize{7}{8}\selectfont},
  cbVerdict/.style={rounded corners=2pt,minimum width=.85cm,minimum height=.34cm,
    font=\sffamily\bfseries\fontsize{7.2}{8.5}\selectfont},
  cbSupported/.style={cbVerdict,fill=cbGreenPale,text=cbGreen},
  cbPartial/.style={cbVerdict,fill=cbAmberPale,text=cbAmber},
  cbNot/.style={cbVerdict,fill=cbRedPale,text=cbRed}
}
\newcommand{\cbHighlight}[2]{\begingroup\setlength{\fboxsep}{1.1pt}\colorbox{#1}{\strut #2}\endgroup}


